A Region-Dependent Gain Condition for Asymptotic Stability

A sufficient condition for the stability of a system resulting from the interconnection of dynamical systems is given by the small gain theorem. Roughly speaking, to apply this theorem, it is required that the gains composition is continuous, increasing and upper bounded by the identity function. In this work, an alternative sufficient condition is presented for the case in which this criterion fails due to either lack of continuity or the bound of the composed gain is larger than the identity function. More precisely, the local (resp. non-local) asymptotic stability of the origin (resp. global attractivity of a compact set) is ensured by a region-dependent small gain condition. Under an additional condition that implies convergence of solutions for almost all initial conditions in a suitable domain, the almost global asymptotic stability of the origin is ensured. Two examples illustrate and motivate this approach.

==> commands.tex <==

% To redeclare a MathOperator: begin
\makeatletter
\newcommand\RedeclareMathOperator{%
  \@ifstar{\def\rmo@s{m}\rmo@redeclare}{\def\rmo@s{o}\rmo@redeclare}%
}
% this is taken from \renew@command
\newcommand\rmo@redeclare[2]{%
  \begingroup \escapechar\m@ne\xdef\@gtempa{{\string#1}}\endgroup
  \expandafter\@ifundefined\@gtempa
     {\@latex@error{\noexpand#1undefined}\@ehc}%
     \relax
  \expandafter\rmo@declmathop\rmo@s{#1}{#2}}
% This is just \@declmathop without \@ifdefinable
\newcommand\rmo@declmathop[3]{%
  \DeclareRobustCommand{#2}{\qopname\newmcodes@#1{#3}}%
}
\@onlypreamble\RedeclareMathOperator
\makeatother
% end %

% Commands with x

\newcommand{\dx}{\dot{x}}
\newcommand{\dy}{\dot{y}}
\newcommand{\xp}{x^+}
\newcommand{\lloc}{\mathcal{L}_\mathrm{loc}}
\newcommand{\cl}{\mathtt{cl}}
\newcommand{\dom}{\mathtt{dom}}
\newcommand{\im}{\mathtt{im}}
\newcommand{\OSC}{\mathcal{OSC}}
\newcommand{\AC}{\mathcal{AC}}
\newcommand{\supp}{\mathtt{supp}}
\newcommand{\MAF}{\mathtt{MAF}}
\newcommand{\id}{\mathtt{id}}
\newcommand{\conv}{\mathtt{conv}}
\newcommand{\sign}{\mathtt{sign}}
\newcommand{\Liploc}{\cL\mathpzc{ip}_\mathrm{loc}}
\newcommand{\Ploc}{\mathcal{P}_{\mathrm{loc}}}
\renewcommand{\ae}{\mathrm{for\ a.e.\ }}

\newcommand{\pfrac}[2]{\raisebox{1pt}{\small \ensuremath{#1}}$/$\raisebox{-2pt}{\small \ensuremath{#2}}}

\DeclareMathOperator{\diag}{\mathtt{diag}}
\DeclareMathOperator{\dist}{\mathtt{dist}}
\DeclareMathOperator{\diverg}{\mathtt{div}}
\RedeclareMathOperator{\div}{\mathtt{div}}
\DeclareMathOperator{\sat}{\mathtt{sat}}

\DeclareMathOperator{\interior}{\mathtt{int}}
\DeclareMathOperator{\ext}{\mathtt{ext}}
\DeclareMathOperator{\dir}{\mathrm{dir}}
\DeclareMathOperator{\gph}{\mathrm{gph}}
\DeclareMathOperator{\card}{\mathtt{card}}
\DeclareMathOperator{\diam}{\mathtt{diam}}
\DeclareMathOperator{\co}{\mathtt{co}}
\DeclareMathOperator{\mes}{\mathtt{mes}}
\DeclareMathOperator{\vol}{\mathtt{vol}}
\DeclareMathOperator{\proj}{\mathtt{proj}}
\DeclareMathOperator{\grad}{\mathtt{grad}}
\DeclareMathOperator*{\esssup}{\mathtt{ess\ sup}}

\newcommand{\new}{\color{black}}
\renewcommand{\stop}{\color{black}}

\newcommand{\blue}{\color{blue}}
\newcommand{\red}{\color{red}}
\newcommand{\black}{\color{black}}
\newcommand{\white}{\color{white}}
\newcommand{\green}{\color{green!50!black}}
\newcommand{\magenta}{\color{magenta}}

